Automatic Annotation of Grammaticality in Child-Caregiver Conversations

The acquisition of grammar has been a central question to adjudicate between theories of language acquisition. In order to conduct faster, more reproducible, and larger-scale corpus studies on grammaticality in child-caregiver conversations, tools for automatic annotation can offer an effective alternative to tedious manual annotation. We propose a coding scheme for context-dependent grammaticality in child-caregiver conversations and annotate more than 4,000 utterances from a large corpus of transcribed conversations. Based on these annotations, we train and evaluate a range of NLP models. Our results show that fine-tuned Transformer-based models perform best, achieving human inter-annotation agreement levels.As a first application and sanity check of this tool, we use the trained models to annotate a corpus almost two orders of magnitude larger than the manually annotated data and verify that children's grammaticality shows a steady increase with age.This work contributes to the growing literature on applying state-of-the-art NLP methods to help study child language acquisition at scale.

==> table2_alt.tex <==

%     \begin{tabular}{p{.12\textwidth}|p{.14\textwidth}p{.24\textwidth}p{.26\textwidth}p{0.11\textwidth}}
% \textbf{Error category (broad)} &\textbf{Error category \newline
% (fine-grained)} & \textbf{Description} & \textbf{Examples} & \textbf{Frequency (Number)} \\
% \midrule
% \multirow[t]{3}{=}{Syntactic } & 
% \texttt{subject} & Missing subject & 
% ``Is hot?'', 
% ``Going there.''
% & 17.7\% (322)
% \\ \cmidrule{2-5}
% & 
% \texttt{object} & Missing object 
% & ``Can we look for.'',
% %``She says.''\newline
% ``I like.'' 
% & 6.4\% (116) 
% \\ \cmidrule{2-5}
% & \texttt{verb} & Missing verb (incl. copula)
% &
% ``This yours.'',
% %``Daddy raisins.''\newline
% ``Because it.''
% & 14.7\% (267) 
% \\
% \midrule
% \multirow[t]{2}{=}{Noun morphology } &
% \texttt{possessive} & Missing or wrong use of possessive 
% & ``What's the other boy name?''\newline
% ``Where is Julia house?''
% &  1.4\% (26) 
% \\ \cmidrule{2-5}
% & 
% \texttt{plural} & Wrong plural form or use & 
% ``No I like mans.'',
% ``More truck.'' 
% &  0.9\% (17)
% \\
% \midrule
% \multirow[t]{2}{=}{Verb morphology } &
% \texttt{sv$\_$agreement} & Subject-verb agreement errors %(incl. 3rd person singular s, to be)
% & 
% ``He want cake.'',
% ``She are happy!'' 
% &  3.4\% (61)
% \\ \cmidrule{2-5}
% & 
% \texttt{tense\_aspect} & Wrong tense or aspect inflection of a verb %(excluding errors with present progressive, these have a separate label)
% &
% %``Did I did it?''\newline
% ``He's forgot me.'', 
% ``She falled over.''
% &  7.9\% (143)
% \\
% \midrule
% \multirow[t]{4}{=}{Unbound morphology} & 
% \texttt{determiner} & Missing or wrong determiner & 
% ``Blue wheel.'',
% %``See window?''\newline
% ``A ice cream?''
% & 18.8\% (342)
% \\ \cmidrule{2-5}
% & \texttt{preposition} & Missing or wrong preposition &
% ``I want see it.'',
% ``Give it me!''
% & 4.1\% (75)
% \\ \cmidrule{2-5}
% & \texttt{auxiliary} & Missing or wrong auxiliary verb &
% ``We not to put them away.'',
% ``Someone been crashed.'' 
% & 11.4\% (207)
% \\ \cmidrule{2-5}
% & \texttt{present$\_$\newline progressive} & Wrong present progressive form& ``It coming.'', ``What's he say?''
% & 4.3\% (78)
% \\
% \midrule
% Other& \texttt{other} & Any other kind of grammatical error &
% ``Many money!'' (many/much)\newline
% ``Why it's falling?'' (word order)\newline
% ``My want to eat'' (wrong case)
% & 8.9\% (162)
% \\
% \end{tabular}



==> table_alt.tex <==


%     \begin{tabular}{p{.04\textwidth}p{.47\textwidth}p{.41\textwidth}}
% \textbf{Label} &\textbf{Cases} & \textbf{Examples} \\
% \midrule
% \multirow[t]{3}{=}[-1em]{\rotatebox[origin=r]{90}{\texttt{\textbf{ungrammatical}}}
% } & Ellipses with missing verb or determiner &
% ``Cookie Monster.'', ``Lunch.'', ``No shoes.''
% \\ \cmidrule{2-3}
% & Ellipses with missing object &
% ''I want.'', ``He gave.''
% \\ \cmidrule{2-3}
% & Ellipses with missing subject, if the context (or verb) clearly points to non-imperative use &
% ``Want to go to the cinema!''
% \\ \cmidrule{2-3}
% &SVO/SV questions (except if they are used as clarification requests or to express surprise)
% &``You are coming (to the house)?''
% \\ \cmidrule{2-3}
% &Ellipses due to the child being interrupted &
% ``I gave.'' - ``That’s great!'' %(As we do not have access to the timing of the utterances, we do not know whether the child was actually interrupted or they just stopped the utterance before completing it. To be consistent, we mark these cases as ungrammatical.)\\
% \\
% \midrule

% \multirow[t]{3}{=}[-6em]{\rotatebox[origin=r]{90}{\texttt{\textbf{ambiguous}}}
% }
% & Onomatopoeia &
% ``Miaow miaow'', ``Muuh muh!'', ``Vroom vroom''
% \\ \cmidrule{2-3}
% & Unknown words or vocalizations, baby language, family-intern expression%, words spontaneously invented by the child 
% &
% %``It’s a planer'', (From the context it’s clear that the child actually means ``pilot'') \newline
% ``Let’s go to the cagriotafer!'', ``eh eh.'' 
% \\ \cmidrule{2-3}
% &Noun phrases that might be grammatical if accompanied with an appropriate gesture, e.g. a pointing gesture towards an object
% &
% ''A zebra!''% (if the determiner is missing (``zebra!'', it should be marked as \texttt{ungrammatical}!)
% , ``For the zebra''
% \\ \cmidrule{2-3}
% &Ellipses with missing subject, for which the context does not clearly discriminate between imperative and declarative use&
% ``Do this.''
% \\ \cmidrule{2-3}
% &Utterances that are grammatically correct, but not aligned with what the child actually intended to say &
% ``That’s a nice cup.'' - ``Is it you?.''\newline% (in this case, the child’s response is grammatical but they most likely intended to say something like ``Is it yours?'', so we annotate it with 0.)\newline
% ``Hide the table'' %(in this case, the child actually meant to say ``Hide under the table''. ``Hide the table'' is strictly speaking grammatical, but we know that there’s actually a grammatical error (missing preposition) if we can infer from the context what the child actually intended to say
% \\ \cmidrule{2-3}
% &Reciting, Singing, Counting &
% ``Sweep, sweep, sweep!'', ``One, two, three.''
% \\ \cmidrule{2-3}
% &Utterances that are strictly ungrammatical but very commonly used in spoken Standard American or British English %errors of omission or subject-verb agreement
% &
% ``Don’t know'', ''You like this?'', ''That all?''
% % ''Know what he did?''
% % ''Remember what we did last Friday''?
% % ``Smells nice.''
% % ``Sounds good.''
% % ``Where’s your boxes?''
% % ``How many women are there?'' - ``There’s two.''
% \\ \cmidrule{2-3}
% &Transcription errors &
% He like’s animals.
% \\

% \midrule
% \multirow[t]{3}{=}[-9em]{\rotatebox[origin=r]{90}{\texttt{\textbf{grammatical}}}
% }
% %& Utterances with missing subject, if they are used as imperatives& Look for it!'', ``Take this.'' \\ \cmidrule{2-3}
% &Utterances with self-repetitions, disfluencies &
% ``I like I like this.'', %``uhm I like it.''
% ``This is uhm a table.''
% % ``This is a, a horse!''
% \\ \cmidrule{2-3}
% &Self-corrections/Reformulations (if the final reformulated utterance is grammatical) &
% ``He want she wants a flower!'' %``She is she was very happy''
% %The case of reformulations across multiple utterances: ``[CHI] He want'' - ``[CHI] She wants a flower'' (The first utterance should be marked as ungrammatical, the second one as grammatical (1)) ``[CHI] She is'' - ``[CHI] She is very clever'' (The first utterance should be marked as ungrammatical (as it is missing an object), the second one as grammatical (1))
% \\ \cmidrule{2-3}
% &Exclamations, backchannels: &
% ``Uh oh.'', ``Mhm hm.'', ``All right.'', ``Oh no!''
% \\ \cmidrule{2-3}
% &Self-repetitions over multiple utterances&
% ``I want an apple.'' - ``An apple.''% (Both utterances should be marked as  grammatical (1))
% \\ \cmidrule{2-3}
% &Repetitions from the previous utterance %as they usually function as positive feedback (except if the child is repeating an erroneous part from a previous utterance
% &
%  %``It is very hot.'' - ``Very hot.''\newline
%  ``This is my funny hat'' - ``My funny hat.''
% %&Repetitions that are e.g. missing a determiner should be marked as ungrammatical & ``[CAR] I like the book'' - ``[CHI] book.''
% \\ \cmidrule{2-3}
% &Ellipses that are valid responses to a question&
% ``Who is that?'' - ``Cookie Monster!''\newline
% % ``What is this?'' - ``The pasta that daddy made yesterday!''
% ``Are you an artist?'' - ``I am.''
% % ``[CAR] Which one is it?'' - ``[CHI] This one.''
% % ''[CAR] what are you going to do?'' - ''[CHI] Run up the stairs.''
% %Note: Usually, questions that ask for a noun (phrase) still require the response to have an appropriate determiner (``[CAR] What is this?'' - ``[CHI] A cat.''). If they are missing the determiner, they should be marked as ungrammatical. However, in case the question directly asks for a concept, a response without a determiner is permitted: ``[CAR] How do we call this?'' - ``[CHI] Cat!''
% %\\ \cmidrule{2-3} &Elliptic follow-up questions:& ``What’s this?'' - ``And that?''
% \\ \cmidrule{2-3}
% &Greetings, calls for attention&
% ''Good Morning.'', 
% ''Mummy, mum!''
% \\ \cmidrule{2-3}
% &Wrong answers, utterances that are logically/semantically wrong or questionable&
%  ``Can you say ‘a rat’?'' - ``A cat!''\newline
%  ``The sky is green.''
% \\ \cmidrule{2-3}
% &Completions of previous utterances&
% ``And then he went'' - ``To the cinema''
% %``These shoes'' - ``Are mine''
% %&Self-completions/expansions over multiple utterances& ``I want.'' - ``This one.'' %(The first utterance should be marked as ungrammatical (as it’s missing an object, the second one as grammatical (1)) ``Where is that?'' - ``At home?''
% \\ \cmidrule{2-3}
% %&SVO/SV questions that function as clarification requests or express surprise & ``This is big.'' - ``This is big?'' \\ \cmidrule{2-3}
% &Short forms/ contractions commonly used in spoken English&
% ``Cause I went to school'', ``You’re sposta go there.'', ``That’s a lotta dogs!'', ``Gotcha!''
% %``Watcha gonna do?'', ``I like ‘em'', ``I was runnin’'', 
% \\ \cmidrule{2-3}
% &Utterances with phonological errors %, either because of dialect or pronunciation difficulties of the child
% &
% ``Sesame Stweet'', ``Dis is a dog''
% % ``Who is dat?'' (instead of ``that'')
% % ``Momma!''
% % ``Let’s go srough this once again.'' (instead of ``through'')
% %(However, if the word is really not recognizable, annotate as ungrammatical)
% \\ \cmidrule{2-3}
% &Ellipses that are clearly accompanied by pointing&
% ``Oh this!'', ``This one.'', ``These cats.''
% \end{tabular}
